Predicting Acute Kidney Injury at Hospital Re-entry Using High-dimensional Electronic Health Record Data

Acute Kidney Injury (AKI), a sudden decline in kidney function, is associated with increased mortality, morbidity, length of stay, and hospital cost. Since AKI is sometimes preventable, there is great interest in prediction. Most existing studies consider all patients and therefore restrict to features available in the first hours of hospitalization. Here, the focus is instead on rehospitalized patients, a cohort in which rich longitudinal features from prior hospitalizations can be analyzed. Our objective is to provide a risk score directly at hospital re-entry. Gradient boosting, penalized logistic regression (with and without stability selection), and a recurrent neural network are trained on two years of adult inpatient EHR data (3,387 attributes for 34,505 patients who generated 90,013 training samples with 5,618 cases and 84,395 controls). Predictions are internally evaluated with 50 iterations of 5-fold grouped cross-validation with special emphasis on calibration, an analysis of which is performed at the patient as well as hospitalization level. Error is assessed with respect to diagnosis, race, age, gender, AKI identification method, and hospital utilization. In an additional experiment, the regularization penalty is severely increased to induce parsimony and interpretability. Predictors identified for rehospitalized patients are also reported with a special analysis of medications that might be modifiable risk factors. Insights from this study might be used to construct a predictive tool for AKI in rehospitalized patients. An accurate estimate of AKI risk at hospital entry might serve as a prior for an admitting provider or another predictive algorithm.

==> old_bib_list_from_orig_sub.tex <==
\begin{thebibliography}{10}

\bibitem{RIFLE2004}
Bellomo R, Ronco C, Kellum JA, Mehta RL, Palevsky P, Acute Dialysis
  Quality~Initiative w.
\newblock Acute renal failure - definition, outcome measures, animal models,
  fluid therapy and information technology needs: the Second International
  Consensus Conference of the Acute Dialysis Quality Initiative (ADQI) Group
  [Journal Article].
\newblock Crit Care. 2004;8(4):R204--12.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/15312219}.

\bibitem{Venkataraman2007}
Venkataraman R, Kellum JA.
\newblock Defining acute renal failure: the RIFLE criteria.
\newblock J Intensive Care Med. 2007;22.
\newblock Available from: \url{http://dx.doi.org/10.1177/0885066607299510}.

\bibitem{chertow2005MortLOSCost}
Chertow GM, Burdick E, Honour M, Bonventre JV, Bates DW.
\newblock Acute kidney injury, mortality, length of stay, and costs in
  hospitalized patients [Journal Article].
\newblock J Am Soc Nephrol. 2005;16(11):3365--70.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/16177006}.

\bibitem{bellomo2012acute}
Bellomo R, Kellum JA, Ronco C.
\newblock Acute kidney injury [Journal Article].
\newblock Lancet. 2012;380(9843):756--66.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/22617274}.

\bibitem{AKIN}
Mehta RL, Kellum JA, Shah SV, Molitoris BA, Ronco C, Warnock DG, et~al.
\newblock Acute Kidney Injury Network: report of an initiative to improve
  outcomes in acute kidney injury [Journal Article].
\newblock Crit Care. 2007;11(2):R31.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/17331245}.

\bibitem{KDIGO-AKIdef2012}
Group KAKIW.
\newblock KDIGO Clinical Practice Guideline for Acute Kidney Injury - Section
  2: AKI Definition [Journal Article].
\newblock Kidney International Supplements;2(1):19--36.
\newblock Available from: \url{http://dx.doi.org/10.1038/kisup.2011.32}.

\bibitem{ERBPpositionState}
Ad-hoc working~group of E, Fliser D, Laville M, Covic A, Fouque D, Vanholder R,
  et~al.
\newblock A European Renal Best Practice (ERBP) position statement on the
  Kidney Disease Improving Global Outcomes (KDIGO) clinical practice guidelines
  on acute kidney injury: part 1: definitions, conservative management and
  contrast-induced nephropathy [Journal Article].
\newblock Nephrol Dial Transplant. 2012;27(12):4263--72.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23045432}.

\bibitem{sutherland2016utilizingAKIADQI}
Sutherland SM, Chawla LS, Kane-Gill SL, Hsu RK, Kramer AA, Goldstein SL, et~al.
\newblock Utilizing electronic health records to predict acute kidney injury
  risk and outcomes: workgroup statements from the 15(th) ADQI Consensus
  Conference [Journal Article].
\newblock Can J Kidney Health Dis. 2016;3:11.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26925247}.

\bibitem{lameire2008prevention}
Lameire N, van Biesen W, Hoste E, Vanholder R.
\newblock The prevention of acute kidney injury an in-depth narrative review:
  Part 2: Drugs in the prevention of acute kidney injury [Journal Article].
\newblock NDT Plus. 2009;2(1):1--10.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25949275}.

\bibitem{TepelPreventContrastRedRenalFunc}
Tepel M, van~der Giet M, Schwarzfeld C, Laufer U, Liermann D, Zidek W.
\newblock Prevention of radiographic-contrast-agent-induced reductions in renal
  function by acetylcysteine [Journal Article].
\newblock N Engl J Med. 2000;343(3):180--4.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/10900277}.

\bibitem{SolomonRadioCon}
Solomon R, Werner C, Mann D, D'Elia J, Silva P.
\newblock Effects of saline, mannitol, and furosemide to prevent acute
  decreases in renal function induced by radiocontrast agents [Journal
  Article].
\newblock N Engl J Med. 1994;331(21):1416--20.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/7969280}.

\bibitem{GuoDrugNephro}
Guo X, Nzerue C.
\newblock How to prevent, recognize, and treat drug-induced nephrotoxicity
  [Journal Article].
\newblock Cleve Clin J Med. 2002;69(4):289--90, 293--4, 296--7 passim.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/11996200}.

\bibitem{VogelzangChemoNeph}
Vogelzang NJ.
\newblock Nephrotoxicity from chemotherapy: prevention and management [Journal
  Article].
\newblock Oncology (Williston Park). 1991;5(10):97--102, 105; disc 105,
  109--11.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/1838278}.

\bibitem{koyner2016development}
Koyner JL, Adhikari R, Edelson DP, Churpek MM.
\newblock Development of a Multicenter Ward-Based AKI Prediction Model [Journal
  Article].
\newblock Clin J Am Soc Nephrol. 2016;11(11):1935--1943.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/27633727}.

\bibitem{calDavis}
Davis SE, Lasko TA, Chen G, Siew ED, Matheny ME.
\newblock Calibration drift in regression and machine learning models for acute
  kidney injury [Journal Article].
\newblock J Am Med Inform Assoc. 2017;Available from:
  \url{https://www.ncbi.nlm.nih.gov/pubmed/28379439}.

\bibitem{CroninVetStrat}
Cronin RM, VanHouten JP, Siew ED, Eden SK, Fihn SD, Nielson CD, et~al.
\newblock National Veterans Health Administration inpatient risk stratification
  models for hospital-acquired acute kidney injury [Journal Article].
\newblock J Am Med Inform Assoc. 2015;22(5):1054--71.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26104740}.

\bibitem{c8}
Kristovic D, Horvatic I, Husedzinovic I, Sutlic Z, Rudez I, Baric D, et~al.
\newblock Cardiac surgery-associated acute kidney injury: risk factors analysis
  and comparison of prediction models [Journal Article].
\newblock Interact Cardiovasc Thorac Surg. 2015;21(3):366--73.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26091696}.

\bibitem{c12}
Tsai TT, Patel UD, Chang TI, Kennedy KF, Masoudi FA, Matheny ME, et~al.
\newblock Validated contemporary risk model of acute kidney injury in patients
  undergoing percutaneous coronary interventions: insights from the National
  Cardiovascular Data Registry Cath-PCI Registry [Journal Article].
\newblock J Am Heart Assoc. 2014;3(6):e001380.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25516439}.

\bibitem{c15}
Gurm HS, Seth M, Kooiman J, Share D.
\newblock A novel tool for reliable and accurate prediction of renal
  complications in patients undergoing percutaneous coronary intervention
  [Journal Article].
\newblock J Am Coll Cardiol. 2013;61(22):2242--8.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23721921}.

\bibitem{c18}
Legrand M, Pirracchio R, Rosa A, Petersen ML, Van~der Laan M, Fabiani JN,
  et~al.
\newblock Incidence, risk factors and prediction of post-operative acute kidney
  injury following cardiac surgery for active infective endocarditis: an
  observational study [Journal Article].
\newblock Crit Care. 2013;17(5):R220.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24093498}.

\bibitem{i1}
Chawla LS, Davison DL, Brasha-Mitchell E, Koyner JL, Arthur JM, Shaw AD, et~al.
\newblock Development and standardization of a furosemide stress test to
  predict the severity of acute kidney injury [Journal Article].
\newblock Crit Care. 2013;17(5):R207.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24053972}.

\bibitem{i2}
Koyner JL, Davison DL, Brasha-Mitchell E, Chalikonda DM, Arthur JM, Shaw AD,
  et~al.
\newblock Furosemide Stress Test and Biomarkers for the Prediction of AKI
  Severity [Journal Article].
\newblock J Am Soc Nephrol. 2015;26(8):2023--31.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25655065}.

\bibitem{i3}
Cruz DN, Ferrer-Nadal A, Piccinni P, Goldstein SL, Chawla LS, Alessandri E,
  et~al.
\newblock Utilization of small changes in serum creatinine with clinical risk
  factors to assess the risk of AKI in critically lll adults [Journal Article].
\newblock Clin J Am Soc Nephrol. 2014;9(4):663--72.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24677553}.

\bibitem{i4}
Forni LG, Dawes T, Sinclair H, Cheek E, Bewick V, Dennis M, et~al.
\newblock Identifying the patient at risk of acute kidney injury: a predictive
  scoring system for the development of acute kidney injury in acute medical
  patients [Journal Article].
\newblock Nephron Clin Pract. 2013;123(3-4):143--50.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23887252}.

\bibitem{i5}
Kane-Gill SL, Sileanu FE, Murugan R, Trietley GS, Handler SM, Kellum JA.
\newblock Risk factors for acute kidney injury in older adults with critical
  illness: a retrospective cohort study [Journal Article].
\newblock Am J Kidney Dis. 2015;65(6):860--9.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25488106}.

\bibitem{i6}
Flechet M, Guiza F, Schetz M, Wouters P, Vanhorebeek I, Derese I, et~al.
\newblock AKIpredictor, an online prognostic calculator for acute kidney injury
  in adult critically ill patients: development, validation and comparison to
  serum neutrophil gelatinase-associated lipocalin [Journal Article].
\newblock Intensive Care Med. 2017;Available from:
  \url{https://www.ncbi.nlm.nih.gov/pubmed/28130688}.

\bibitem{Kate2016}
Kate RJ, Perez RM, Mazumdar D, Pasupathy KS, Nilakantan V.
\newblock Prediction and detection models for acute kidney injury in
  hospitalized older adults.
\newblock BMC Medical Informatics and Decision Making. 2016;16(1):39.
\newblock Available from: \url{http://dx.doi.org/10.1186/s12911-016-0277-4}.

\bibitem{livt2}
Xu X, Ling Q, Wei Q, Wu J, Gao F, He ZL, et~al.
\newblock An effective model for predicting acute kidney injury after liver
  transplantation [Journal Article].
\newblock Hepatobiliary Pancreat Dis Int. 2010;9(3):259--63.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/20525552}.

\bibitem{lungT1}
Grimm JC, Lui C, Kilic A, Valero r V, Sciortino CM, Whitman GJ, et~al.
\newblock A risk score to predict acute renal failure in adult patients after
  lung transplantation [Journal Article].
\newblock Ann Thorac Surg. 2015;99(1):251--7.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25440281}.

\bibitem{R1}
McMahon GM, Zeng X, Waikar SS.
\newblock A risk prediction score for kidney failure or mortality in
  rhabdomyolysis [Journal Article].
\newblock JAMA Intern Med. 2013;173(19):1821--8.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24000014}.

\bibitem{R2}
Rodriguez E, Soler MJ, Rap O, Barrios C, Orfila MA, Pascual J.
\newblock Risk factors for acute kidney injury in severe rhabdomyolysis
  [Journal Article].
\newblock PLoS One. 2013;8(12):e82992.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24367578}.

\bibitem{Breiman_alg_v_mod}
Breiman L, et~al.
\newblock Statistical modeling: The two cultures (with comments and a rejoinder
  by the author).
\newblock Statistical science. 2001;16(3):199--231.

\bibitem{friedman2001greedy}
Friedman JH.
\newblock Greedy function approximation: a gradient boosting machine.
\newblock Annals of statistics. 2001;p. 1189--1232.

\bibitem{tibshirani1996regression}
Tibshirani R.
\newblock Regression shrinkage and selection via the lasso.
\newblock Journal of the Royal Statistical Society Series B (Methodological).
  1996;p. 267--288.

\bibitem{waikar2006validity}
Waikar SS, Wald R, Chertow GM, Curhan GC, Winkelmayer WC, Liangos O, et~al.
\newblock Validity of International Classification of Diseases, Ninth Revision,
  Clinical Modification Codes for Acute Renal Failure [Journal Article].
\newblock J Am Soc Nephrol. 2006;17(6):1688--94.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/16641149}.

\bibitem{lipton2016directly}
Lipton ZC, Kale D, Wetzel R.
\newblock Directly modeling missing data in sequences with RNNs: Improved
  classification of clinical time series.
\newblock In: Machine Learning for Healthcare Conference; 2016. p. 253--270.

\bibitem{singhLeveHier}
Singh A, Nadkarni G, Guttag J, Bottinger E.
\newblock Leveraging hierarchy in medical codes for predictive modeling.
\newblock In: Proceedings of the 5th ACM Conference on Bioinformatics,
  Computational Biology, and Health Informatics. ACM;. p. 96--103.

\bibitem{goldstein2017comparison}
Goldstein BA, Pomann GM, Winkelmayer WC, Pencina MJ.
\newblock A comparison of risk prediction methods using repeated observations:
  an application to electronic health records for hemodialysis.
\newblock Statistics in Medicine. 2017;.

\bibitem{choiHF}
Choi E, Schuetz A, Stewart WF, Sun J.
\newblock Using recurrent neural network models for early detection of heart
  failure onset.
\newblock Journal of the American Medical Informatics Association.
  2017;24(2):361.
\newblock Available from: \url{+ http://dx.doi.org/10.1093/jamia/ocw112}.

\bibitem{colopy2017bayesian}
Colopy GW, Roberts S, Clifton D.
\newblock Bayesian Optimisation of Personalised Models for Patient Vital-Sign
  Monitoring.
\newblock IEEE Journal of Biomedical and Health Informatics. 2017;.

\bibitem{alaa2016hidden}
Alaa AM, van~der Schaar M.
\newblock A Hidden Absorbing Semi-Markov Model for Informatively Censored
  Temporal Data: Learning and Inference.
\newblock arXiv preprint arXiv:161206007. 2016;.

\bibitem{cawley2010over}
Cawley GC, Talbot NL.
\newblock On over-fitting in model selection and subsequent selection bias in
  performance evaluation.
\newblock Journal of Machine Learning Research. 2010;11(Jul):2079--2107.

\bibitem{varma2006bias}
Varma S, Simon R.
\newblock Bias in error estimation when using cross-validation for model
  selection.
\newblock BMC bioinformatics. 2006;7(1):91.

\bibitem{bergstra2012random}
Bergstra J, Bengio Y.
\newblock Random search for hyper-parameter optimization.
\newblock Journal of Machine Learning Research. 2012;13(Feb):281--305.

\bibitem{hoerl1970ridge}
Hoerl AE, Kennard RW.
\newblock Ridge regression: Biased estimation for nonorthogonal problems.
\newblock Technometrics. 1970;12(1):55--67.

\bibitem{Breiman_RF}
Breiman L.
\newblock Random forests [Journal Article].
\newblock Machine Learning. 2001;45(1):5--32.
\newblock Available from: \url{<Go to ISI>://WOS:000170489900001}.

\bibitem{rumelhart1985learning}
Rumelhart DE, Hinton GE, Williams RJ.
\newblock Learning internal representations by error propagation.
\newblock California Univ San Diego La Jolla Inst for Cognitive Science; 1985.

\bibitem{harrell2015regression}
Harrell F.
\newblock Regression modeling strategies: with applications to linear models,
  logistic and ordinal regression, and survival analysis.
\newblock Springer; 2015.

\bibitem{Platt}
Platt J, et~al.
\newblock Probabilistic outputs for support vector machines and comparisons to
  regularized likelihood methods.
\newblock Advances in large margin classifiers. 1999;10(3):61--74.

\bibitem{caruana2015intelligible}
Caruana R, Lou Y, Gehrke J, Koch P, Sturm M, Elhadad N.
\newblock Intelligible models for healthcare: Predicting pneumonia risk and
  hospital 30-day readmission.
\newblock In: Proceedings of the 21th ACM SIGKDD International Conference on
  Knowledge Discovery and Data Mining. ACM; 2015. p. 1721--1730.

\bibitem{KCraw}
Crawford K.
\newblock The Trouble with Bias.
\newblock NIPS 2017, Long Beach, CA.; 2017. Available from:
  \url{https://nips.cc/Conferences/2017/Schedule?showEvent=8742}.

\bibitem{corbett2017algorithmic}
Corbett-Davies S, Pierson E, Feller A, Goel S, Huq A.
\newblock Algorithmic decision making and the cost of fairness.
\newblock arXiv preprint arXiv:170108230. 2017;.

\bibitem{pedregosa2011scikit}
Pedregosa F, Varoquaux G, Gramfort A, Michel V, Thirion B, Grisel O, et~al.
\newblock Scikit-learn: Machine Learning in Python [Journal Article].
\newblock Journal of Machine Learning Research. 2011;12(Oct):2825--2830.
\newblock Available from: \url{<Go to ISI>://WOS:000298103200003}.

\bibitem{scipy}
Jones E, Oliphant T, Peterson P, et~al.. {SciPy}: Open source scientific tools
  for {Python}; 2001--.
\newblock [Online; accessed <today>].
\newblock Available from: \url{http://www.scipy.org/}.

\bibitem{mckinney2010pandas}
McKinney W.
\newblock Data structures for statistical computing in python.
\newblock In: Proceedings of the 9th Python in Science Conference. vol. 445.
  van der Voort S, Millman J;. p. 51--56.

\bibitem{perez2007ipython}
Pérez F, Granger BE.
\newblock IPython: a system for interactive scientific computing [Journal
  Article].
\newblock Computing in Science and Engineering. 2007;9(3).

\bibitem{Hunter:2007}
Hunter JD.
\newblock Matplotlib: A 2D graphics environment.
\newblock Computing In Science \& Engineering. 2007;9(3):90--95.

\bibitem{behnel2010cython}
Behnel S, Bradshaw R, Citro C, Dalcin L, Seljebotn DS, Smith K.
\newblock Cython: The Best of Both Worlds.
\newblock Computing in Science Engineering. 2011;13(2):31 --39.

\bibitem{walt2011numpy}
Walt Svd, Colbert SC, Varoquaux G.
\newblock The NumPy array: a structure for efficient numerical computation.
\newblock Computing in Science \& Engineering. 2011;13(2):22--30.

\bibitem{ShustermanHospAcq}
Shusterman N, Strom BL, Murray TG, Morrison G, West SL, Maislin G.
\newblock Risk factors and outcome of hospital-acquired acute renal failure.
  Clinical epidemiologic study [Journal Article].
\newblock Am J Med. 1987;83(1):65--71.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/3605183}.

\bibitem{chawla2014acute}
Chawla LS, Eggers PW, Star RA, Kimmel PL.
\newblock Acute kidney injury and chronic kidney disease as interconnected
  syndromes.
\newblock New England Journal of Medicine. 2014;371(1):58--66.

\bibitem{ronco2008cardiorenal}
Ronco C, Haapio M, House AA, Anavekar N, Bellomo R.
\newblock Cardiorenal syndrome.
\newblock Journal of the American College of Cardiology.
  2008;52(19):1527--1539.

\bibitem{LeblancRiskFact}
Leblanc M, Kellum JA, Gibney RT, Lieberthal W, Tumlin J, Mehta R.
\newblock Risk factors for acute renal failure: inherent and modifiable risks
  [Journal Article].
\newblock Curr Opin Crit Care. 2005;11(6):533--6.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/16292055}.

\bibitem{garcia2008acute}
Garcia-Tsao G, Parikh CR, Viola A.
\newblock Acute kidney injury in cirrhosis.
\newblock Hepatology. 2008;48(6):2064--2077.

\bibitem{fede2012renal}
Fede G, D’Amico G, Arvaniti V, Tsochatzis E, Germani G, Georgiadis D, et~al.
\newblock Renal failure and cirrhosis: a systematic review of mortality and
  prognosis.
\newblock Journal of hepatology. 2012;56(4):810--818.

\bibitem{PalevskyCommentOnKDIGONephConsult}
Palevsky PM, Liu KD, Brophy PD, Chawla LS, Parikh CR, Thakar CV, et~al.
\newblock KDOQI US commentary on the 2012 KDIGO clinical practice guideline for
  acute kidney injury [Journal Article].
\newblock Am J Kidney Dis. 2013;61(5):649--72.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23499048}.

\bibitem{Futoma_comp_readmis}
Futoma J, Morris J, Lucas J.
\newblock A comparison of models for predicting early hospital readmissions
  [Journal Article].
\newblock J Biomed Inform. 2015;56:229--38.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26044081}.

\bibitem{icd9com}
ICD9Data.com;.
\newblock \url{http://www.icd9data.com}.

\bibitem{ERvisit2014}
Ryan K, Levit K, Davis PH.
\newblock Characteristics of Weekday and Weekend Hospital Admissions.
\newblock Rockville, MD: Agency for Healthcare Research and Quality; 2010. 87.

\bibitem{naesens2009calcineurin}
Naesens M, Kuypers DR, Sarwal M.
\newblock Calcineurin inhibitor nephrotoxicity.
\newblock Clinical Journal of the American Society of Nephrology.
  2009;4(2):481--508.

\bibitem{leite2015renal}
Leite TT, Macedo E, da~Silva~Martins I, de~Oliveira~Neves FM, Lib{\'o}rio AB.
\newblock Renal outcomes in critically ill patients receiving propofol or
  midazolam.
\newblock Clinical Journal of the American Society of Nephrology. 2015;p.
  CJN--02330315.

\bibitem{atici2004opioid}
Atici S, Cinel L, Cinel I, Doruk N, Aktekin M, Akca A, et~al.
\newblock Opioid neurotoxicity: comparison of morphine and tramadol in an
  experimental rat model.
\newblock International Journal of Neuroscience. 2004;114(8):1001--1011.

\bibitem{shmueli2010explain}
Shmueli G, et~al.
\newblock To explain or to predict?
\newblock Statistical science. 2010;25(3):289--310.

\bibitem{callahan2018machine}
Callahan A, Shah NH.
\newblock Machine Learning in Healthcare.
\newblock In: Key Advances in Clinical Informatics. Elsevier; 2018. p.
  279--291.

\bibitem{BengioReg}
Jo J, Bengio Y.
\newblock Measuring the tendency of CNNs to Learn Surface Statistical
  Regularities.
\newblock arXiv preprint arXiv:171111561. 2017;.

\bibitem{doi:10.1001/jama.2017.19198}
A V, NH S, RA H.
\newblock What this computer needs is a physician: Humanism and artificial
  intelligence.
\newblock JAMA. 2017;Available from: \url{+
  http://dx.doi.org/10.1001/jama.2017.19198}.

\bibitem{choi2016multi}
Choi E, Bahadori MT, Searles E, Coffey C, Thompson M, Bost J, et~al.
\newblock Multi-layer representation learning for medical concepts.
\newblock In: Proceedings of the 22nd ACM SIGKDD International Conference on
  Knowledge Discovery and Data Mining. ACM; 2016. p. 1495--1504.

\bibitem{gbcSK}
Scikit-learn Gradient Boosting Classifier;.
\newblock
  \url{http://scikit-learn.org/stable/modules/generated/sklearn.ensemble.GradientBoostingClassifier.html}.

\bibitem{LR1SK}
Scikit-learn Logistic Regression;.
\newblock
  \url{http://scikit-learn.org/stable/modules/generated/sklearn.linear_model.LogisticRegression.html}.

\bibitem{LassoSK}
Scikit-learn Lasso;.
\newblock
  \url{http://scikit-learn.org/stable/modules/generated/sklearn.linear_model.Lasso.html}.

\end{thebibliography}

==> predicting-aki-project-13 1/old_bib_list_from_orig_sub.tex <==
\begin{thebibliography}{10}

\bibitem{RIFLE2004}
Bellomo R, Ronco C, Kellum JA, Mehta RL, Palevsky P, Acute Dialysis
  Quality~Initiative w.
\newblock Acute renal failure - definition, outcome measures, animal models,
  fluid therapy and information technology needs: the Second International
  Consensus Conference of the Acute Dialysis Quality Initiative (ADQI) Group
  [Journal Article].
\newblock Crit Care. 2004;8(4):R204--12.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/15312219}.

\bibitem{Venkataraman2007}
Venkataraman R, Kellum JA.
\newblock Defining acute renal failure: the RIFLE criteria.
\newblock J Intensive Care Med. 2007;22.
\newblock Available from: \url{http://dx.doi.org/10.1177/0885066607299510}.

\bibitem{chertow2005MortLOSCost}
Chertow GM, Burdick E, Honour M, Bonventre JV, Bates DW.
\newblock Acute kidney injury, mortality, length of stay, and costs in
  hospitalized patients [Journal Article].
\newblock J Am Soc Nephrol. 2005;16(11):3365--70.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/16177006}.

\bibitem{bellomo2012acute}
Bellomo R, Kellum JA, Ronco C.
\newblock Acute kidney injury [Journal Article].
\newblock Lancet. 2012;380(9843):756--66.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/22617274}.

\bibitem{AKIN}
Mehta RL, Kellum JA, Shah SV, Molitoris BA, Ronco C, Warnock DG, et~al.
\newblock Acute Kidney Injury Network: report of an initiative to improve
  outcomes in acute kidney injury [Journal Article].
\newblock Crit Care. 2007;11(2):R31.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/17331245}.

\bibitem{KDIGO-AKIdef2012}
Group KAKIW.
\newblock KDIGO Clinical Practice Guideline for Acute Kidney Injury - Section
  2: AKI Definition [Journal Article].
\newblock Kidney International Supplements;2(1):19--36.
\newblock Available from: \url{http://dx.doi.org/10.1038/kisup.2011.32}.

\bibitem{ERBPpositionState}
Ad-hoc working~group of E, Fliser D, Laville M, Covic A, Fouque D, Vanholder R,
  et~al.
\newblock A European Renal Best Practice (ERBP) position statement on the
  Kidney Disease Improving Global Outcomes (KDIGO) clinical practice guidelines
  on acute kidney injury: part 1: definitions, conservative management and
  contrast-induced nephropathy [Journal Article].
\newblock Nephrol Dial Transplant. 2012;27(12):4263--72.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23045432}.

\bibitem{sutherland2016utilizingAKIADQI}
Sutherland SM, Chawla LS, Kane-Gill SL, Hsu RK, Kramer AA, Goldstein SL, et~al.
\newblock Utilizing electronic health records to predict acute kidney injury
  risk and outcomes: workgroup statements from the 15(th) ADQI Consensus
  Conference [Journal Article].
\newblock Can J Kidney Health Dis. 2016;3:11.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26925247}.

\bibitem{lameire2008prevention}
Lameire N, van Biesen W, Hoste E, Vanholder R.
\newblock The prevention of acute kidney injury an in-depth narrative review:
  Part 2: Drugs in the prevention of acute kidney injury [Journal Article].
\newblock NDT Plus. 2009;2(1):1--10.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25949275}.

\bibitem{TepelPreventContrastRedRenalFunc}
Tepel M, van~der Giet M, Schwarzfeld C, Laufer U, Liermann D, Zidek W.
\newblock Prevention of radiographic-contrast-agent-induced reductions in renal
  function by acetylcysteine [Journal Article].
\newblock N Engl J Med. 2000;343(3):180--4.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/10900277}.

\bibitem{SolomonRadioCon}
Solomon R, Werner C, Mann D, D'Elia J, Silva P.
\newblock Effects of saline, mannitol, and furosemide to prevent acute
  decreases in renal function induced by radiocontrast agents [Journal
  Article].
\newblock N Engl J Med. 1994;331(21):1416--20.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/7969280}.

\bibitem{GuoDrugNephro}
Guo X, Nzerue C.
\newblock How to prevent, recognize, and treat drug-induced nephrotoxicity
  [Journal Article].
\newblock Cleve Clin J Med. 2002;69(4):289--90, 293--4, 296--7 passim.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/11996200}.

\bibitem{VogelzangChemoNeph}
Vogelzang NJ.
\newblock Nephrotoxicity from chemotherapy: prevention and management [Journal
  Article].
\newblock Oncology (Williston Park). 1991;5(10):97--102, 105; disc 105,
  109--11.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/1838278}.

\bibitem{koyner2016development}
Koyner JL, Adhikari R, Edelson DP, Churpek MM.
\newblock Development of a Multicenter Ward-Based AKI Prediction Model [Journal
  Article].
\newblock Clin J Am Soc Nephrol. 2016;11(11):1935--1943.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/27633727}.

\bibitem{calDavis}
Davis SE, Lasko TA, Chen G, Siew ED, Matheny ME.
\newblock Calibration drift in regression and machine learning models for acute
  kidney injury [Journal Article].
\newblock J Am Med Inform Assoc. 2017;Available from:
  \url{https://www.ncbi.nlm.nih.gov/pubmed/28379439}.

\bibitem{CroninVetStrat}
Cronin RM, VanHouten JP, Siew ED, Eden SK, Fihn SD, Nielson CD, et~al.
\newblock National Veterans Health Administration inpatient risk stratification
  models for hospital-acquired acute kidney injury [Journal Article].
\newblock J Am Med Inform Assoc. 2015;22(5):1054--71.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26104740}.

\bibitem{c8}
Kristovic D, Horvatic I, Husedzinovic I, Sutlic Z, Rudez I, Baric D, et~al.
\newblock Cardiac surgery-associated acute kidney injury: risk factors analysis
  and comparison of prediction models [Journal Article].
\newblock Interact Cardiovasc Thorac Surg. 2015;21(3):366--73.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26091696}.

\bibitem{c12}
Tsai TT, Patel UD, Chang TI, Kennedy KF, Masoudi FA, Matheny ME, et~al.
\newblock Validated contemporary risk model of acute kidney injury in patients
  undergoing percutaneous coronary interventions: insights from the National
  Cardiovascular Data Registry Cath-PCI Registry [Journal Article].
\newblock J Am Heart Assoc. 2014;3(6):e001380.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25516439}.

\bibitem{c15}
Gurm HS, Seth M, Kooiman J, Share D.
\newblock A novel tool for reliable and accurate prediction of renal
  complications in patients undergoing percutaneous coronary intervention
  [Journal Article].
\newblock J Am Coll Cardiol. 2013;61(22):2242--8.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23721921}.

\bibitem{c18}
Legrand M, Pirracchio R, Rosa A, Petersen ML, Van~der Laan M, Fabiani JN,
  et~al.
\newblock Incidence, risk factors and prediction of post-operative acute kidney
  injury following cardiac surgery for active infective endocarditis: an
  observational study [Journal Article].
\newblock Crit Care. 2013;17(5):R220.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24093498}.

\bibitem{i1}
Chawla LS, Davison DL, Brasha-Mitchell E, Koyner JL, Arthur JM, Shaw AD, et~al.
\newblock Development and standardization of a furosemide stress test to
  predict the severity of acute kidney injury [Journal Article].
\newblock Crit Care. 2013;17(5):R207.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24053972}.

\bibitem{i2}
Koyner JL, Davison DL, Brasha-Mitchell E, Chalikonda DM, Arthur JM, Shaw AD,
  et~al.
\newblock Furosemide Stress Test and Biomarkers for the Prediction of AKI
  Severity [Journal Article].
\newblock J Am Soc Nephrol. 2015;26(8):2023--31.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25655065}.

\bibitem{i3}
Cruz DN, Ferrer-Nadal A, Piccinni P, Goldstein SL, Chawla LS, Alessandri E,
  et~al.
\newblock Utilization of small changes in serum creatinine with clinical risk
  factors to assess the risk of AKI in critically lll adults [Journal Article].
\newblock Clin J Am Soc Nephrol. 2014;9(4):663--72.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24677553}.

\bibitem{i4}
Forni LG, Dawes T, Sinclair H, Cheek E, Bewick V, Dennis M, et~al.
\newblock Identifying the patient at risk of acute kidney injury: a predictive
  scoring system for the development of acute kidney injury in acute medical
  patients [Journal Article].
\newblock Nephron Clin Pract. 2013;123(3-4):143--50.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23887252}.

\bibitem{i5}
Kane-Gill SL, Sileanu FE, Murugan R, Trietley GS, Handler SM, Kellum JA.
\newblock Risk factors for acute kidney injury in older adults with critical
  illness: a retrospective cohort study [Journal Article].
\newblock Am J Kidney Dis. 2015;65(6):860--9.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25488106}.

\bibitem{i6}
Flechet M, Guiza F, Schetz M, Wouters P, Vanhorebeek I, Derese I, et~al.
\newblock AKIpredictor, an online prognostic calculator for acute kidney injury
  in adult critically ill patients: development, validation and comparison to
  serum neutrophil gelatinase-associated lipocalin [Journal Article].
\newblock Intensive Care Med. 2017;Available from:
  \url{https://www.ncbi.nlm.nih.gov/pubmed/28130688}.

\bibitem{Kate2016}
Kate RJ, Perez RM, Mazumdar D, Pasupathy KS, Nilakantan V.
\newblock Prediction and detection models for acute kidney injury in
  hospitalized older adults.
\newblock BMC Medical Informatics and Decision Making. 2016;16(1):39.
\newblock Available from: \url{http://dx.doi.org/10.1186/s12911-016-0277-4}.

\bibitem{livt2}
Xu X, Ling Q, Wei Q, Wu J, Gao F, He ZL, et~al.
\newblock An effective model for predicting acute kidney injury after liver
  transplantation [Journal Article].
\newblock Hepatobiliary Pancreat Dis Int. 2010;9(3):259--63.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/20525552}.

\bibitem{lungT1}
Grimm JC, Lui C, Kilic A, Valero r V, Sciortino CM, Whitman GJ, et~al.
\newblock A risk score to predict acute renal failure in adult patients after
  lung transplantation [Journal Article].
\newblock Ann Thorac Surg. 2015;99(1):251--7.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/25440281}.

\bibitem{R1}
McMahon GM, Zeng X, Waikar SS.
\newblock A risk prediction score for kidney failure or mortality in
  rhabdomyolysis [Journal Article].
\newblock JAMA Intern Med. 2013;173(19):1821--8.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24000014}.

\bibitem{R2}
Rodriguez E, Soler MJ, Rap O, Barrios C, Orfila MA, Pascual J.
\newblock Risk factors for acute kidney injury in severe rhabdomyolysis
  [Journal Article].
\newblock PLoS One. 2013;8(12):e82992.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/24367578}.

\bibitem{Breiman_alg_v_mod}
Breiman L, et~al.
\newblock Statistical modeling: The two cultures (with comments and a rejoinder
  by the author).
\newblock Statistical science. 2001;16(3):199--231.

\bibitem{friedman2001greedy}
Friedman JH.
\newblock Greedy function approximation: a gradient boosting machine.
\newblock Annals of statistics. 2001;p. 1189--1232.

\bibitem{tibshirani1996regression}
Tibshirani R.
\newblock Regression shrinkage and selection via the lasso.
\newblock Journal of the Royal Statistical Society Series B (Methodological).
  1996;p. 267--288.

\bibitem{waikar2006validity}
Waikar SS, Wald R, Chertow GM, Curhan GC, Winkelmayer WC, Liangos O, et~al.
\newblock Validity of International Classification of Diseases, Ninth Revision,
  Clinical Modification Codes for Acute Renal Failure [Journal Article].
\newblock J Am Soc Nephrol. 2006;17(6):1688--94.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/16641149}.

\bibitem{lipton2016directly}
Lipton ZC, Kale D, Wetzel R.
\newblock Directly modeling missing data in sequences with RNNs: Improved
  classification of clinical time series.
\newblock In: Machine Learning for Healthcare Conference; 2016. p. 253--270.

\bibitem{singhLeveHier}
Singh A, Nadkarni G, Guttag J, Bottinger E.
\newblock Leveraging hierarchy in medical codes for predictive modeling.
\newblock In: Proceedings of the 5th ACM Conference on Bioinformatics,
  Computational Biology, and Health Informatics. ACM;. p. 96--103.

\bibitem{goldstein2017comparison}
Goldstein BA, Pomann GM, Winkelmayer WC, Pencina MJ.
\newblock A comparison of risk prediction methods using repeated observations:
  an application to electronic health records for hemodialysis.
\newblock Statistics in Medicine. 2017;.

\bibitem{choiHF}
Choi E, Schuetz A, Stewart WF, Sun J.
\newblock Using recurrent neural network models for early detection of heart
  failure onset.
\newblock Journal of the American Medical Informatics Association.
  2017;24(2):361.
\newblock Available from: \url{+ http://dx.doi.org/10.1093/jamia/ocw112}.

\bibitem{colopy2017bayesian}
Colopy GW, Roberts S, Clifton D.
\newblock Bayesian Optimisation of Personalised Models for Patient Vital-Sign
  Monitoring.
\newblock IEEE Journal of Biomedical and Health Informatics. 2017;.

\bibitem{alaa2016hidden}
Alaa AM, van~der Schaar M.
\newblock A Hidden Absorbing Semi-Markov Model for Informatively Censored
  Temporal Data: Learning and Inference.
\newblock arXiv preprint arXiv:161206007. 2016;.

\bibitem{cawley2010over}
Cawley GC, Talbot NL.
\newblock On over-fitting in model selection and subsequent selection bias in
  performance evaluation.
\newblock Journal of Machine Learning Research. 2010;11(Jul):2079--2107.

\bibitem{varma2006bias}
Varma S, Simon R.
\newblock Bias in error estimation when using cross-validation for model
  selection.
\newblock BMC bioinformatics. 2006;7(1):91.

\bibitem{bergstra2012random}
Bergstra J, Bengio Y.
\newblock Random search for hyper-parameter optimization.
\newblock Journal of Machine Learning Research. 2012;13(Feb):281--305.

\bibitem{hoerl1970ridge}
Hoerl AE, Kennard RW.
\newblock Ridge regression: Biased estimation for nonorthogonal problems.
\newblock Technometrics. 1970;12(1):55--67.

\bibitem{Breiman_RF}
Breiman L.
\newblock Random forests [Journal Article].
\newblock Machine Learning. 2001;45(1):5--32.
\newblock Available from: \url{<Go to ISI>://WOS:000170489900001}.

\bibitem{rumelhart1985learning}
Rumelhart DE, Hinton GE, Williams RJ.
\newblock Learning internal representations by error propagation.
\newblock California Univ San Diego La Jolla Inst for Cognitive Science; 1985.

\bibitem{harrell2015regression}
Harrell F.
\newblock Regression modeling strategies: with applications to linear models,
  logistic and ordinal regression, and survival analysis.
\newblock Springer; 2015.

\bibitem{Platt}
Platt J, et~al.
\newblock Probabilistic outputs for support vector machines and comparisons to
  regularized likelihood methods.
\newblock Advances in large margin classifiers. 1999;10(3):61--74.

\bibitem{caruana2015intelligible}
Caruana R, Lou Y, Gehrke J, Koch P, Sturm M, Elhadad N.
\newblock Intelligible models for healthcare: Predicting pneumonia risk and
  hospital 30-day readmission.
\newblock In: Proceedings of the 21th ACM SIGKDD International Conference on
  Knowledge Discovery and Data Mining. ACM; 2015. p. 1721--1730.

\bibitem{KCraw}
Crawford K.
\newblock The Trouble with Bias.
\newblock NIPS 2017, Long Beach, CA.; 2017. Available from:
  \url{https://nips.cc/Conferences/2017/Schedule?showEvent=8742}.

\bibitem{corbett2017algorithmic}
Corbett-Davies S, Pierson E, Feller A, Goel S, Huq A.
\newblock Algorithmic decision making and the cost of fairness.
\newblock arXiv preprint arXiv:170108230. 2017;.

\bibitem{pedregosa2011scikit}
Pedregosa F, Varoquaux G, Gramfort A, Michel V, Thirion B, Grisel O, et~al.
\newblock Scikit-learn: Machine Learning in Python [Journal Article].
\newblock Journal of Machine Learning Research. 2011;12(Oct):2825--2830.
\newblock Available from: \url{<Go to ISI>://WOS:000298103200003}.

\bibitem{scipy}
Jones E, Oliphant T, Peterson P, et~al.. {SciPy}: Open source scientific tools
  for {Python}; 2001--.
\newblock [Online; accessed <today>].
\newblock Available from: \url{http://www.scipy.org/}.

\bibitem{mckinney2010pandas}
McKinney W.
\newblock Data structures for statistical computing in python.
\newblock In: Proceedings of the 9th Python in Science Conference. vol. 445.
  van der Voort S, Millman J;. p. 51--56.

\bibitem{perez2007ipython}
Pérez F, Granger BE.
\newblock IPython: a system for interactive scientific computing [Journal
  Article].
\newblock Computing in Science and Engineering. 2007;9(3).

\bibitem{Hunter:2007}
Hunter JD.
\newblock Matplotlib: A 2D graphics environment.
\newblock Computing In Science \& Engineering. 2007;9(3):90--95.

\bibitem{behnel2010cython}
Behnel S, Bradshaw R, Citro C, Dalcin L, Seljebotn DS, Smith K.
\newblock Cython: The Best of Both Worlds.
\newblock Computing in Science Engineering. 2011;13(2):31 --39.

\bibitem{walt2011numpy}
Walt Svd, Colbert SC, Varoquaux G.
\newblock The NumPy array: a structure for efficient numerical computation.
\newblock Computing in Science \& Engineering. 2011;13(2):22--30.

\bibitem{ShustermanHospAcq}
Shusterman N, Strom BL, Murray TG, Morrison G, West SL, Maislin G.
\newblock Risk factors and outcome of hospital-acquired acute renal failure.
  Clinical epidemiologic study [Journal Article].
\newblock Am J Med. 1987;83(1):65--71.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/3605183}.

\bibitem{chawla2014acute}
Chawla LS, Eggers PW, Star RA, Kimmel PL.
\newblock Acute kidney injury and chronic kidney disease as interconnected
  syndromes.
\newblock New England Journal of Medicine. 2014;371(1):58--66.

\bibitem{ronco2008cardiorenal}
Ronco C, Haapio M, House AA, Anavekar N, Bellomo R.
\newblock Cardiorenal syndrome.
\newblock Journal of the American College of Cardiology.
  2008;52(19):1527--1539.

\bibitem{LeblancRiskFact}
Leblanc M, Kellum JA, Gibney RT, Lieberthal W, Tumlin J, Mehta R.
\newblock Risk factors for acute renal failure: inherent and modifiable risks
  [Journal Article].
\newblock Curr Opin Crit Care. 2005;11(6):533--6.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/16292055}.

\bibitem{garcia2008acute}
Garcia-Tsao G, Parikh CR, Viola A.
\newblock Acute kidney injury in cirrhosis.
\newblock Hepatology. 2008;48(6):2064--2077.

\bibitem{fede2012renal}
Fede G, D’Amico G, Arvaniti V, Tsochatzis E, Germani G, Georgiadis D, et~al.
\newblock Renal failure and cirrhosis: a systematic review of mortality and
  prognosis.
\newblock Journal of hepatology. 2012;56(4):810--818.

\bibitem{PalevskyCommentOnKDIGONephConsult}
Palevsky PM, Liu KD, Brophy PD, Chawla LS, Parikh CR, Thakar CV, et~al.
\newblock KDOQI US commentary on the 2012 KDIGO clinical practice guideline for
  acute kidney injury [Journal Article].
\newblock Am J Kidney Dis. 2013;61(5):649--72.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/23499048}.

\bibitem{Futoma_comp_readmis}
Futoma J, Morris J, Lucas J.
\newblock A comparison of models for predicting early hospital readmissions
  [Journal Article].
\newblock J Biomed Inform. 2015;56:229--38.
\newblock Available from: \url{https://www.ncbi.nlm.nih.gov/pubmed/26044081}.

\bibitem{icd9com}
ICD9Data.com;.
\newblock \url{http://www.icd9data.com}.

\bibitem{ERvisit2014}
Ryan K, Levit K, Davis PH.
\newblock Characteristics of Weekday and Weekend Hospital Admissions.
\newblock Rockville, MD: Agency for Healthcare Research and Quality; 2010. 87.

\bibitem{naesens2009calcineurin}
Naesens M, Kuypers DR, Sarwal M.
\newblock Calcineurin inhibitor nephrotoxicity.
\newblock Clinical Journal of the American Society of Nephrology.
  2009;4(2):481--508.

\bibitem{leite2015renal}
Leite TT, Macedo E, da~Silva~Martins I, de~Oliveira~Neves FM, Lib{\'o}rio AB.
\newblock Renal outcomes in critically ill patients receiving propofol or
  midazolam.
\newblock Clinical Journal of the American Society of Nephrology. 2015;p.
  CJN--02330315.

\bibitem{atici2004opioid}
Atici S, Cinel L, Cinel I, Doruk N, Aktekin M, Akca A, et~al.
\newblock Opioid neurotoxicity: comparison of morphine and tramadol in an
  experimental rat model.
\newblock International Journal of Neuroscience. 2004;114(8):1001--1011.

\bibitem{shmueli2010explain}
Shmueli G, et~al.
\newblock To explain or to predict?
\newblock Statistical science. 2010;25(3):289--310.

\bibitem{callahan2018machine}
Callahan A, Shah NH.
\newblock Machine Learning in Healthcare.
\newblock In: Key Advances in Clinical Informatics. Elsevier; 2018. p.
  279--291.

\bibitem{BengioReg}
Jo J, Bengio Y.
\newblock Measuring the tendency of CNNs to Learn Surface Statistical
  Regularities.
\newblock arXiv preprint arXiv:171111561. 2017;.

\bibitem{doi:10.1001/jama.2017.19198}
A V, NH S, RA H.
\newblock What this computer needs is a physician: Humanism and artificial
  intelligence.
\newblock JAMA. 2017;Available from: \url{+
  http://dx.doi.org/10.1001/jama.2017.19198}.

\bibitem{choi2016multi}
Choi E, Bahadori MT, Searles E, Coffey C, Thompson M, Bost J, et~al.
\newblock Multi-layer representation learning for medical concepts.
\newblock In: Proceedings of the 22nd ACM SIGKDD International Conference on
  Knowledge Discovery and Data Mining. ACM; 2016. p. 1495--1504.

\bibitem{gbcSK}
Scikit-learn Gradient Boosting Classifier;.
\newblock
  \url{http://scikit-learn.org/stable/modules/generated/sklearn.ensemble.GradientBoostingClassifier.html}.

\bibitem{LR1SK}
Scikit-learn Logistic Regression;.
\newblock
  \url{http://scikit-learn.org/stable/modules/generated/sklearn.linear_model.LogisticRegression.html}.

\bibitem{LassoSK}
Scikit-learn Lasso;.
\newblock
  \url{http://scikit-learn.org/stable/modules/generated/sklearn.linear_model.Lasso.html}.

\end{thebibliography}
